TopViewRS: Vision-Language Models as Top-View Spatial Reasoners

Top-view perspective denotes a typical way in which humans read and reason over different types of maps, and it is vital for localization and navigation of humans as well as of `non-human' agents, such as the ones backed by large Vision-Language Models (VLMs). Nonetheless, spatial reasoning capabilities of modern VLMs remain unattested and underexplored. In this work, we thus study their capability to understand and reason over spatial relations from the top view. The focus on top view also enables controlled evaluations at different granularity of spatial reasoning; we clearly disentangle different abilities (e.g., recognizing particular objects versus understanding their relative positions). We introduce the TopViewRS (Top-View Reasoning in Space) dataset, consisting of 11,384 multiple-choice questions with either realistic or semantic top-view map as visual input. We then use it to study and evaluate VLMs across 4 perception and reasoning tasks with different levels of complexity. Evaluation of 10 representative open- and closed-source VLMs reveals the gap of more than 50% compared to average human performance, and it is even lower than the random baseline in some cases. Although additional experiments show that Chain-of-Thought reasoning can boost model capabilities by 5.82% on average, the overall performance of VLMs remains limited. Our findings underscore the critical need for enhanced model capability in top-view spatial reasoning and set a foundation for further research towards human-level proficiency of VLMs in real-world multimodal tasks.

==> table/data_examples.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|c|l}
\hline
\textbf{Sub-Task}                          & \textbf{Measuring Ability}                    & \textbf{Example}                                                                                                                                                 \\ \hline
\multirow{4}{*}{Top-View Understanding}    & \multirow{2}{*}{Object Recognition}           & \begin{tabular}[c]{@{}l@{}}Which of the following objects are in the room?\\ A. shelving; B. bed; C. toilet; D. seating;\end{tabular}                            \\
                                           &                                               & \begin{tabular}[c]{@{}l@{}}Which of the following objects are not in the room?\\ A. sink; B. table; C. toilet; D. cushion;\end{tabular}                          \\ \cline{2-3} 
                                           & \multirow{2}{*}{Scene Recognition}            & \begin{tabular}[c]{@{}l@{}}What room is this?\\ A. entryway/foyer/lobby; B. bedroom; C. toilet; D. bathroom;\end{tabular}                                        \\
                                           &                                               & \begin{tabular}[c]{@{}l@{}}What types of rooms are included in the top-view map below?\\ A. balcony; B. lounge; C. bedroom; D. laundryroom/mudroom;\end{tabular} \\ \hline
\multirow{3}{*}{Spatial Understanding}     & Object Spatial Understanding                  & \begin{tabular}[c]{@{}l@{}}Where is the bed in the top-down map?\\ A. middle center; B. bottom left; C. middle right; D. top right;\end{tabular}                 \\ \cline{2-3} 
                                           & \multirow{2}{*}{Scene Spatial Understanding}  & \begin{tabular}[c]{@{}l@{}}What objects does bedroom have? \\ A. gym\_equipment; B. sofa; C. plant; D. chest\_of\_drawers;\end{tabular}                          \\
                                           &                                               & \begin{tabular}[c]{@{}l@{}}Where is the bedroom in the top-down map?\\ A. top left; B. middle center; C. bottom right; D. middle right;\end{tabular}             \\ \hline
\multirow{3}{*}{Spatial Reasoning}         & Scene Counting                                & \begin{tabular}[c]{@{}l@{}}How many bedroom are there? \\ A. 0; B. 1; C. 2; D. 3\end{tabular}                                                                    \\ \cline{2-3} 
                                           & \multirow{2}{*}{Relative Spatial Relation}    & \begin{tabular}[c]{@{}l@{}}What's bed's relative spatial relations to cushion? \\ A. up right; B. down left; C. overlap; D. down right;\end{tabular}             \\
                                           &                                               & \begin{tabular}[c]{@{}l@{}}What's bedroom's relative spatial relation to bathroom? \\ A. up left; B. up right; C. down right; D. down left;\end{tabular}         \\ \hline
\multirow{5}{*}{Dynamic Spatial Reasoning} & Dynamic Action Counting                       & \begin{tabular}[c]{@{}l@{}}How many turning left are there along the path? \\ A. 1; B. 2; C. 4; D. 3;\end{tabular}                                               \\ \cline{2-3} 
                                           & \multirow{3}{*}{Dynamic Spatial Localization} & \begin{tabular}[c]{@{}l@{}}What rooms does the navigation path pass by?\\ A. living room; B. utilityroom/toolroom; C. balcony; D. kitchen;\end{tabular}          \\
                                           &                                               & \begin{tabular}[c]{@{}l@{}}At which room does the navigation path start? \\ A. porch/terrace/deck; B. living room; C. stairs; D. balcony;\end{tabular}           \\
                                           &                                               & \begin{tabular}[c]{@{}l@{}}At which object does the navigation path stop? \\ A. stool; B. counter; C. lighting; D. door;\end{tabular}                            \\ \cline{2-3} 
                                           & Dynamic Relative Spatial Relation             & \begin{tabular}[c]{@{}l@{}}Which direction does the navigation path head for?\\ A. up right; B. down left; C. right; D. left;\end{tabular}                       \\ \hline
\end{tabular}%
}
\caption{}
\label{tab:dataset example}
\end{table*}
